Mixed Laplace approximation for marginal posterior and Bayesian inference in error-in-operator model

Laplace approximation is a very useful tool in Bayesian inference and it claims a nearly Gaussian behavior of the posterior. \cite{SpLaplace2022} established some rather accurate finite sample results about the quality of Laplace approximation in terms of the so called effective dimension $p$ under the critical dimension constraint $p^{3} \ll n$. However, this condition can be too restrictive for many applications like error-in-operator problem or Deep Neuronal Networks. This paper addresses the question whether the dimensionality condition can be relaxed and the accuracy of approximation can be improved if the target of estimation is low dimensional while the nuisance parameter is high or infinite dimensional. Under mild conditions, the marginal posterior can be approximated by a Gaussian mixture and the accuracy of the approximation only depends on the target dimension. Under the condition $p^{2} \ll n$ or in some special situation like semi-orthogonality, the Gaussian mixture can be replaced by one Gaussian distribution leading to a classical Laplace result. The second result greatly benefits from the recent advances in Gaussian comparison from \cite{GNSUl2017}. The results are illustrated and specified for the case of error-in-operator model.

==> genMLE.tex <==
% !TEX root = ../generic.tex

%\ifapp{} % for appendix
%{ % for main part
\Chapter{Properties of the pMLE \( \tilde{\upsv}_{\GP} \)}
\label{SgenBounds}
This \chname collects general results about concentration and expansion of the pMLE
%The use of self-concordance conditions from Section~\ref{Slocalsmooth} helps to 
which substantially improve the bounds from \cite{SpPa2019}.
% and about Gaussian approximation of the posterior that can be used in many situations. 
%
We assume to be given a pseudo log-likelihood random function \( L(\upsv) \), \( \upsv \in \Ups \subseteq \R^{\dimp} \),
\( \dimp < \infty \).
Given a quadratic penalty \( \| \GP \upsv \|^{2}/2 \), define 
\begin{EQA}
	\LGP(\upsv) 
	&=& 
	L(\upsv) - \| \GP \upsv \|^{2}/2 .
\label{LGLum2Gu22}
\end{EQA}
Typical examples of choosing \( \GP^{2} \) are given in Section~\ref{Ssmoothprior}.
Consider the penalized MLE \( \tilde{\upsv}_{\GP} \) and its population counterpart \( \upsvs_{\GP} \)
\begin{EQA}[rcccl]
	\tilde{\upsv}_{\GP} 
	&=& 
	\argmax_{\upsv} \LGP(\upsv),
	\qquad
	\upsvs_{\GP} 
	&=& 
	\argmax_{\upsv} \E \LGP(\upsv). 
\label{tuGauLGususGE}
\end{EQA}
The corresponding Fisher information matrix \( \IF_{\GP}(\upsv) \) is given by 
\begin{EQA}[rcccl]
	\IF(\upsv) 
	&=& 
	- \nabla^{2} \E L(\upsv) ,
	\qquad
	\IF_{\GP}(\upsv) 
	&=& 
	- \nabla^{2} \E \LGP(\upsv) 
	= 
	\IF(\upsv) + \GP^{2} .
\label{e456yhgfr567uhgf}
\end{EQA}
We assume \( \IF_{\GP}(\upsv) \) to be positive definite for all considered \( \upsv \). 
By \( \DPGP(\upsv) \) we denote a positive symmetric matrix with \( \DPGP^{2}(\upsv) = \IF_{\GP}(\upsv) \), and
\( \IF_{\GP} = \IF_{\GP}(\upsvs_{\GP}) \), \( \DPGP = \IF_{\GP}^{1/2} \). 

%
\Section{Conditions}
\label{Scondgeneric}
Now we present our conditions.
The most important one is about linearity of the stochastic component 
\( \zeta(\upsv) = L(\upsv) - \E L(\upsv) = \LGP(\upsv) - \E \LGP(\upsv) \).

\begin{description}
    \item[\label{Eref} \( \bb{(\zeta)} \)]
      \textit{The stochastic component \( \zeta(\upsv) = L(\upsv) - \E L(\upsv) \) of the process \( L(\upsv) \) is linear in 
      \( \upsv \). We denote by \( \nabla \zeta \equiv \nabla \zeta(\upsv) \in \R^{\dimp} \) its gradient
      }.
  \end{description}


Below we assume some concentration properties of the stochastic vector \( \nabla \zeta \).
%
More precisely, we require that \( \nabla \zeta \) obeys the following condition;
see \eqref{PxivbzzBBroB3} of Theorem~\ref{Tdevboundgm}.
\begin{description}
\item[\label{EU2ref}\( \bb{(\nabla \zeta)} \)]
	\textit{Let \( \VP^{2} = \Var(\nabla \zeta) \) and 
	\( \DPGP^{2} = \DPGP^{2}(\upsvs_{\GP}) \).
	Then for any considered \( \xx > 0 \)
	}
\begin{EQA}
	\P\bigl( \| \DPGP^{-1} \nabla \zeta \| \geq \rr_{\GP}(\xx) \bigr)
	& \leq &
	3 \ex^{-\xx} ,
\label{2emxGPm12nz122}
\end{EQA}
where for \( \dimG = \tr(\DPGP^{-2} \VP^{2}) \) and \( \lambda_{\GP} = \| \DPGP^{-1} \VP^{2} \DPGP^{-1} \| \)
\begin{EQA}
	\rr_{\GP}(\xx)
	& \eqdef &
	\sqrt{\dimG} + \sqrt{2 \xx \lambda_{\GP}} \,  .
\label{34rtyghuioiuyhgvftid}
\end{EQA}
\end{description}

This condition can be effectively checked if the errors in the data exhibit sub-Gaussian or sub-exponential behaviour;
see Section~\ref{SdevboundnonGauss}.
The important value \( \dimG = \tr(\DPGP^{-2} \VP^{2}) \) can be called the \emph{effective dimension}; see \cite{SP2013_rough}.

We also assume that the deterministic part \( \E \LGP(\upsv) \) 
of the penalized log-likelihood is a concave function.
It can be relaxed using localization; see \cite{Sp2019NLI}.
%In particular, the result below about
%concentration of the pMLE \( \tilde{\upsv}_{\GP} \) assumes concavity of \( \E \LGP(\upsv) \).
\begin{description}
    \item[\label{LLref} \( \bb{(\mathcal{C}_{\GP})} \)]
      \textit{\( \Ups \) is an open and convex set in \( \R^{\dimp} \).
        The function \( \E \LGP(\upsv) \) is concave on \( \Ups \).        
      }
\end{description}

\ifLaplace{
In Section~\ref{Spostconcentr} we consider a stronger condition of semi-concavity of \( \E L(\upsv) \). }{}
%
Further we will also need some smoothness conditions on the function \( f(\upsv) = \E L(\upsv) \).
The class of models satisfying the conditions \nameref{Eref}, 
\nameref{EU2ref}
with a smooth function \( f(\upsv) = \E L(\upsv) \) will be referred to as \emph{stochastically linear smooth} (SLS). 
This class includes linear regression, generalized linear models (GLM) and log-density models; 
see \cite{SpPa2019}\ifapp{ or Section~\ref{SGBvM} later.}{.}
However, this class is much larger.
For instance, nonlinear regression and nonlinear inverse problems can be adapted to the SLS framework 
by an extension of the parameter space; see \cite{Sp2019NLI}.



\Section{Concentration of the pMLE \( \tilde{\upsv}_{\GP} \)}
\label{SgenpMLE}
%\Section {Properties of the pMLE \( \tilde{\upsv}_{\GP} \)}
This section discusses some concentration properties of the pMLE \( \tilde{\upsv}_{\GP} = \argmax_{\upsv} \LGP(\upsv) \).
%around the point \( \upsvs_{\GP} \).
%It is worth mentioning that the concentration bounds only rely on the basic conditions 
%\nameref{Eref},
%\nameref{EU2ref},
%\nameref{LLref},
%and on the local smoothness properties of the function \( f(\upsv) = \E L(\upsv) \) in the Gateaux sense.

Given \( \xx \) and \( \rr_{\GP} = \rr_{\GP}(\xx) \) from \eqref{34rtyghuioiuyhgvftid}, define for some \( \amax < 1 \) the set \( \UVz_{\GP} \) by
\begin{EQA}
	\UVz_{\GP}
	& \eqdef &
	\bigl\{ \uv \colon \| \DPGP \uv \| \leq \amax^{-1} \rr_{\GP} \bigr\} .
\label{rm1ucDGu2r0DGu}
\end{EQA}
%
The result of this section states the concentration properties of the pMLE \( \tilde{\upsv}_{\GP} \)
in the local vicinity \( \CA_{\GP} \) of \( \upsvs_{\GP} \) of the form 
\begin{EQA}
	\CA_{\GP}
	& \eqdef &
	\upsvs_{\GP} + \UVz_{\GP}
	=
	\bigl\{ \upsv = \upsvs_{\GP} + \uv \colon \uv \in \UVz_{\GP} \bigr\}
	\subseteq \Upsd .
\label{UsuvcruvusGiV0}
\end{EQA}
Local Gateaux-regularity of \( f(\upsv) = \E L(\upsv) \) within \( \CA_{\GP} \)
will be measured by the error of the second order Taylor approximation
\begin{EQ}[rcl]
	\dltw_{3}(\upsv,\uv) 
	&=& 
	f(\upsv + \uv) - f(\upsv) - \langle \nabla f(\upsv), \uv \rangle 
	- \frac{1}{2} \langle \nabla^{2} f(\upsv), \uv^{\otimes 2} \rangle , 
	\\
	\dltwd_{3}(\upsv,\uv) 
	&=&
	\langle \nabla f(\upsv + \uv), \uv \rangle - \langle \nabla f(\upsv), \uv \rangle 
	- \langle \nabla^{2} f(\upsv), \uv^{\otimes 2} \rangle \, .
\label{dltw3vufuv12f2g}
\end{EQ}
More precisely, %as in \eqref{dtb3u1DG2d3GPg} with \( \upsv = \upsvs_{\GP} \) and \( \HLG(\upsv) = \DPGP \), 
define
\begin{EQA}
    \dltwb_{\GP}
    & \eqdef &
    \sup_{\uv \in \UVz_{\GP}}
    \frac{2 |\dltw_{3}(\upsvs_{\GP},\uv)|}{\| \DPGP \uv \|^{2}} \,\, ,
    \qquad
    \dltwbd_{\GP}
    \eqdef 
    \sup_{\uv \in \UVz_{\GP}} \frac{2 |\dltwd_{3}(\upsvs_{\GP},\uv)|}{\| \DPGP \uv \|^{2}} \,\, . 
\label{dtb3u1DG2d3GP}
\end{EQA}
The quantities \( \dltwb_{\GP} \) and \( \dltwbd_{\GP} \) can be effectively bounded under smoothness
conditions \nameref{LL3tref} or \nameref{LLtS3ref} given in Section~\ref{Slocalsmooth}.
Under \nameref{LL3tref} at \( \upsv = \upsvs_{\GP} \) with \( \DVL^{2}(\upsvs_{\GP}) = \DPGP^{2} \)
and \( \rr = \rrGP \), by Lemma~\ref{LdltwLa3t}, it holds for a small constant \( \dltwu_{3} \)
\begin{EQA}
	\dltwbd_{\GP}
	& \leq &
	\dltwu_{3} \, \amax^{-1} \rrGP \, ,
	\qquad
	\dltwb_{\GP}
	\leq 
	\dltwu_{3} \, \amax^{-1} \rrGP/ 3 .
\label{swdy6fwqd6qtxcvbdyfdtw}
\end{EQA}
Furthermore, under \nameref{LLtS3ref}, the same bounds apply with \( \dltwu_{3} = \hmax_{3} n^{-1/2} \); see Lemma~\ref{LdltwLaGP}.


\begin{proposition}
\label{PconcMLEgenc}
Suppose
\nameref{Eref},
\nameref{EU2ref},
%\nameref{LL0ref},
and %let \( \E \LGP(\upsv) \) be a concave function. 
\nameref{LLref}.
Let also %\( \dltwbd_{\GP} \) from \eqref{dtb3u1DG2d3GP} and \( \amax \) from \eqref{rm1ucDGu2r0DGu} fulfill
%and all \( \uv \) with \( \amax \DPGP \uv \in \UVz \)
\begin{EQA}
	1 - \amax - \dltwbd_{\GP}
	& \geq &
	0 ;
\label{rrm23r0ut3u}
\end{EQA}
see \eqref{dtb3u1DG2d3GP} and \eqref{rm1ucDGu2r0DGu}.
Then \( \tilde{\upsv}_{\GP} \in \CA_{\GP} \) on a set \( \Omega(\xx) \) with \( \P\bigl( \Omega(\xx) \bigr) \geq 1 - 3 \ex^{-\xx} \), 
i.e.
\begin{EQA}
	\| \DPGP (\tilde{\upsv}_{\GP} - \upsvs_{\GP}) \|  
	& \leq &
	\amax^{-1} \rrGP \, . 
\label{rhDGtuGmusGU0}
\end{EQA}
\end{proposition}

\begin{proof}
By \nameref{EU2ref}, on a the random set \( \Omega(\xx) \) with 
\( \P(\Omega(\xx)) \geq 1 - 3 \ex^{-\xx} \), it holds \( \| \DPGP^{-1} \nabla \zeta \| \leq \rr_{\GP} \).
Now the result follows from Proposition~\ref{Pconcgeneric} with 
\( \fs(\upsv) = \E \LGP(\upsv) \), \( \fn(\upsv) = \LGP(\upsv) \), \( \rrn = \amax^{-1} \rrGP \), and \( \Av = \nabla \zeta \).
\end{proof}

\begin{remark}
The result \eqref{rhDGtuGmusGU0} continues to apply with any matrix 
\( \DU \) in place of \( \DPGP \) provided that 
\( \DU \leq \DPGP \) and \nameref{EU2ref} as well as \eqref{dtb3u1DG2d3GP}, \eqref{rrm23r0ut3u} hold after this change.
\end{remark}

\ifsupnorm{\input sourceB/nanonorm}{}


\Section{Fisher and Wilks expansions}
\label{SFiWiexs}
This section presents some finite sample results about the behavior of the penalized MLE 
\( \tilde{\upsv}_{\GP} \) and the excess \( \LGP(\tilde{\upsv}_{\GP}) - \LGP(\upsvs_{\GP}) \).
Proposition~\ref{PconcMLEgenc} 
states the concentration properties of \( \tilde{\upsv}_{\GP} \) around \( \upsvs_{\GP} \).
Now we show that this concentration can be used to establish a version of the Fisher expansion for 
the estimation error \( \tilde{\upsv}_{\GP} - \upsvs_{\GP} \) and the Wilks expansion for the excess 
\( L_{\GP}(\tilde{\upsv}_{\GP}) - L_{\GP}(\upsvs_{\GP}) \).
%Let \( \dltwb_{\GP} \) be defined by \eqref{dta3u1DG2sr}.

\begin{theorem}
\label{TFiWititG}
Assume the conditions of 
Proposition~\ref{PconcMLEgenc}
%and let \( \dltwb_{\GP} \leq 1/3 \); see \eqref{dtb3u1DG2d3GP}.
with \( \amax = 2/3 \).
Then on \( \Omega(\xx) \!\) 
\begin{EQ}[rcl]
    2 \LGP(\tilde{\upsv}_{\GP}) - 2 \LGP(\upsvs_{\GP}) 
    - \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2}
    & \leq &
    \frac{\dltwb_{\GP}}{1 - \dltwb_{\GP}} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2} \, ,
    \\
    2 \LGP(\tilde{\upsv}_{\GP}) - 2 \LGP(\upsvs_{\GP}) 
    - \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2}
    & \geq &
    - \dltwb_{\GP} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2} .
\label{3d3Af12DGttG}
\end{EQ}
Also
\begin{EQ}[rcl]
    \bigl\| \DPGP \bigl( \tilde{\upsv}_{\GP} - \upsvs_{\GP} \bigr) - \DPGP^{-1} \nabla \zeta \bigr\|^{2}
    & \leq &
    \frac{3 \dltwb_{\GP}}{(1 - \dltwb_{\GP})^{2}} \, \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2} \, ,
%\label{DGttGtsGDGm13rG}
    \\
    \bigl\| \DPGP \bigl( \tilde{\upsv}_{\GP} - \upsvs_{\GP} \bigr) \bigr\|
    & \leq &
    \frac{1 + \sqrt{2 \dltwb_{\GP}}}{1 - \dltwb_{\GP}} \, \bigl\| \DPGP^{-1} \nabla \zeta \bigr\| \, .
\label{DGttGtsGDGm13rG}
\end{EQ}
%
\end{theorem}

%\Section{Proof of Theorem~\ref{TFiWititG}}
\begin{proof}
The result follows from Proposition~\ref{PFiWigeneric} similarly to Proposition~\ref{PconcMLEgenc}.
%By Proposition~\ref{PconcMLEgenc}, on the random set \( \Omega(\xx) \) of dominating probability, the estimate
%\( \tilde{\upsv}_{\GP} \) belongs to the set \( \CA_{\GP} \) yielding 
%\( \tilde{\upsv}_{\GP} - \upsvs_{\GP} \in \UVz_{\GP} \).
%By definition of \( \upsvs_{\GP} = \argmax_{\upsv} \E \LGP(\upsv) \), it holds
%\( \nabla \E \LGP(\upsvs_{\GP}) = 0 \).
%Furthermore, \( \nabla^{2} \E \LGP(\upsvs_{\GP}) = - \DPGP^{2} \).
%%For any \( \upsv \in \CA_{\GP} \), the difference \( \uv = \upsv - \upsvs_{\GP} \) satisfies 
%%\( \uv \in \UVz \).
%By \eqref{dtb3u1DG2d3GP}, for any \( \upsv \in \CA_{\GP} \)
%\begin{EQA}
%	\Bigl| 
%		\E \LGP(\upsvs_{\GP}) - \E \LGP(\upsv) - \frac{1}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) \bigr\|^{2} 
%	\Bigr|
%	& \leq &
%	\frac{\dltwb_{\GP}}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) \bigr\|^{2} .
%\label{d3GrGELGtsG12}
%\end{EQA}
%Further, 
%\begin{EQ}[rcl]
%	&& \nquad
%	\LGP(\upsv) - \LGP(\upsvs_{\GP}) - \frac{1}{2} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2}
%	\\
%	&=&
%	\bigl\langle \upsv - \upsvs_{\GP}, \nabla \zeta \bigr\rangle
%	+ \E \LGP(\upsv) - \E \LGP(\upsvs_{\GP}) - \frac{1}{2} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2} 
%	\\
%	&=&
%	- \frac{1}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) - \DPGP^{-1} \nabla \zeta \bigr\|^{2}
%	+ \E \LGP(\upsv) - \E \LGP(\upsvs_{\GP}) + \frac{1}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) \bigr\|^{2} .
%	\qquad 
%\label{12ELGuELusG}
%\end{EQ}
%As \( \tilde{\upsv}_{\GP} \in \CA_{\GP} \) and it maximizes \( \LGP(\upsv) \), we derive by \eqref{d3GrGELGtsG12}
%\begin{EQA}
%	&& \nquad
%	\LGP(\tilde{\upsv}_{\GP}) - \LGP(\upsvs_{\GP}) - \frac{1}{2} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2}
%	=
%	\max_{\upsv \in \CA_{\GP}} 
%	\Bigl\{ 
%		\LGP(\upsv) - \LGP(\upsvs_{\GP}) - \frac{1}{2} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2} 
%	\Bigr\}
%	\\
%	& \leq &
%	\max_{\upsv \in \CA_{\GP}} 
%	\Bigl\{ 
%		- \frac{1}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) - \DPGP^{-1} \nabla \zeta \bigr\|^{2} 
%		+ \frac{\dltwb_{\GP}}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) \bigr\|^{2}
%	\Bigr\} .
%\label{d3G1212222B} 
%\end{EQA}
%Further, \( \max_{\uv} \bigl\{ \tau \| \uv \|^{2} - \| \uv - \xiv \|^{2} \bigr\} = \frac{\tau}{1 - \tau} \| \xiv \|^{2} \)
%for any \( \tau \in [0,1] \) and \( \xiv \in \R^{\dimp} \), 
%yielding
%\begin{EQA}
%	\LGP(\tilde{\upsv}_{\GP}) - \LGP(\upsvs_{\GP}) - \frac{1}{2} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2}
%	& \leq &
%	\frac{\dltwb_{\GP}}{2(1 - \dltwb_{\GP})} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2} . 
%\label{fd3G122B2} 
%\end{EQA}
%Similarly 
%\begin{EQA}
%	&& \nquad
%	\LGP(\tilde{\upsv}_{\GP}) - \LGP(\upsvs_{\GP}) - \frac{1}{2} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2}
%	\\
%	& \geq &
%	\max_{\upsv \in \CA_{\GP}} 
%	\Bigl\{ 
%		- \frac{1}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) - \DPGP^{-1} \nabla \zeta \bigr\|^{2} 
%		- \frac{\dltwb_{\GP}}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) \bigr\|^{2}
%	\Bigr\}
%	\\
%	&=&
%	- \frac{\dltwb_{\GP} }{2(1 + \dltwb_{\GP})} \, \| \DPGP^{-1} \nabla \zeta \|^{2} . 
%	\qquad \quad
%\label{fd3G122B2m} 
%\end{EQA}
%These bounds imply %as \eqref{DGttGtsGDGm13rG} as 
%\eqref{3d3Af12DGttG}.
%
%Now we derive similarly to \eqref{12ELGuELusG} that for \( \upsv \in \CA_{\GP} \)
%\begin{EQA}
%	\LGP(\upsv) - \LGP(\upsvs_{\GP}) 
%	& \leq &
%	\bigl\langle \upsv - \upsvs_{\GP}, \nabla \zeta \bigr\rangle
%	- \frac{1 - \dltwb_{\GP}}{2} \bigl\| \DPGP (\upsv - \upsvs_{\GP}) \bigr\|^{2} .
%\label{LGvLGvsGf1d3G2}
%\end{EQA}
%A particular choice \( \upsv = \tilde{\upsv}_{\GP} \) yields
%\begin{EQA}
%	\LGP(\tilde{\upsv}_{\GP}) - \LGP(\upsvs_{\GP}) 
%	& \leq &
%	\bigl\langle \tilde{\upsv}_{\GP} - \upsvs_{\GP}, \nabla \zeta \bigr\rangle
%	- \frac{1 - \dltwb_{\GP}}{2} \bigl\| \DPGP (\tilde{\upsv}_{\GP} - \upsvs_{\GP}) \bigr\|^{2} .
%\label{21GsvtvGDG3G2}
%\end{EQA}
%Combining with \eqref{fd3G122B2m} allows to bound
%\begin{EQA}
%	&& \nquad
%	\bigl\langle \tilde{\upsv}_{\GP} - \upsvs_{\GP}, \nabla \zeta \bigr\rangle
%	- \frac{1 - \dltwb_{\GP}}{2} \bigl\| \DPGP (\tilde{\upsv}_{\GP} - \upsvs_{\GP}) \bigr\|^{2} 
%	- \frac{1}{2} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2}
%%	\\
%%	& \geq &
%	\geq 
%	- \frac{\dltwb_{\GP}}{2(1 + \dltwb_{\GP})} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|^{2} .
%\label{2m1DGd3G123G}
%\end{EQA}
%%
%Further, for \( \xiv = \DPGP^{-1} \nabla \zeta \), 
%\( \uv = \DPGP (\tilde{\upsv}_{\GP} - \upsvs_{\GP}) \), and 
%\( \dltwu = \dltwb_{\GP} \in [0,1/3] \), the inequality 
%\begin{EQA}
%	2 \bigl\langle \uv, \xiv \bigr\rangle - (1 - \dltwu) \| \uv \|^{2} - \| \xiv \|^{2}
%	& \geq &
%	- \frac{\dltwu}{1 + \dltwu} \| \xiv \|^{2} 
%\label{dtxi2fd1d22}
%\end{EQA}
%implies 
%\begin{EQA}
%	\bigl\| \uv - \frac{1}{1-\dltwu} \xiv \bigr\|^{2}
%	& \leq &
%	\frac{2 \dltwu}{(1 + \dltwu) (1 - \dltwu)^{2}} \| \xiv \|^{2}
%\label{uv11wxi22w1w}
%\end{EQA}
%yielding for \( \dltwu \leq 1/3 \)
%\begin{EQA}
%	\| \uv - \xiv \|
%	& \leq &
%	\biggl( \dltwu + \sqrt{\frac{2 \dltwu}{1 + \dltwu}} \biggr)
%	\frac{\| \xiv \|}{1 - \dltwu}
%	\leq 
%	\frac{\sqrt{3 \dltwu} \| \xiv \|}{1 - \dltwu} \, ,
%	\\
%	\| \uv \|
%	& \leq &
%	\biggl( 1 + \sqrt{\frac{2 \dltwu}{1 + \dltwu}} \biggr)
%	\frac{\| \xiv \|}{1 - \dltwu}
%	\leq 
%	\frac{1 + \sqrt{2 \dltwu} \| \xiv \|}{1 - \dltwu} \, ,
%\label{uxiBws2w1w31w}
%\end{EQA}
%and \eqref{DGttGtsGDGm13rG} follows.
\end{proof}

%} % end of ifapp

\Section{Effective sample size and critical dimension in pMLE}
\label{ScritdimMLE}
This section discusses the important question of the critical parameter dimension 
still ensuring the validity of the presented results.
A very important feature of our results is their dimension free and coordinate free form.
The true parametric dimension \( \dimp \) can be very large, it does not show up in the error terms.
Neither do we use any spectral decomposition or sequence space structure, in particular, we do not require that 
the Fisher information matrix \( \IF \) and the penalty matrix \( \GP^{2} \) are diagonal or can be jointly diagonalized. 
The results are stated for the general data \( \Yv \) and a quasi log-likelihood function.
In particular, we do not assume independent or progressively dependent observations and additive structure 
of the log-likelihood. 
The \emph{effective sample size} \( \nsize \) can be defined via the smallest eigenvalue of the matrix 
\( \IF_{\GP} = \DPGP^{2} = - \nabla^{2} \E \LGP(\upsvs_{\GP}) \):
\begin{EQA}
	n^{-1}
	& \eqdef &
	\| \IF_{\GP}^{-1} \| .
\label{ikdfu4rdu7yr47gfurkj}
\end{EQA}
%Moreover, if the \( Y_{i} \)'s are i.i.d. then \( \IF(\upsv) \) is proportional to \( n \).
Our results apply as long as this value is sufficiently small. 
%One may also interpret the value \( n \) in \eqref{ikdfu4rdu7yr47gfurkj} as \emph{signal strength}.
%
In typical examples like regression or density modeling
%\ifapp{\Chname \ref{Saniligot} and \Chname \ref{SGBvM}}
%{\Chname \ref{SGBvM}}
%we will see that 
such defined value is closely related to the sample size of the data.

For the concentration result of Proposition~\ref{PconcMLEgenc}
we need the basic conditions \nameref{Eref} and \nameref{LLref}.
Further, \nameref{EU2ref} identifies the radius \( \rrGP \) of the local vicinity \( \CA_{\GP} \).
The final critical condition is given by \eqref{rrm23r0ut3u}.
Essentially it says that the values \( \dltwb_{\GP} \) and \( \dltwbd_{\GP} \) are significantly smaller than 1. 
%We focus on the \( \ell_{2} \)-setup of Section~\ref{Snanonorm} with the local set \( \UVz_{\GP} \) from \eqref{rm1ucDGu2r0DGu}. 
Under \nameref{LLtS3ref}, \( \dltwbd_{\GP} %\leq \CONST \rr_{\GP} \| \DPGP^{-1} \| 
\leq \hmax_{3} \, \amax^{-1} \rr_{\GP} \, \nsize^{-1/2} \); see Lemma~\ref{LdltwLaGP}.
% or Section~\ref{Saniligot} for more details for the GLM case.
So,  
\eqref{rrm23r0ut3u} means \( \rr_{\GP}^{2} \ll \nsize \).
Moreover, definition \eqref{2emxGPm12nz122} of \( \rr_{\GP} \) yields that 
\( \rr_{\GP}^{2} \asymp \tr(\DPGP^{-2} \VP^{2}) = \dimVG \), where \( \dimVG \) is the \emph{effective dimension} of the problem.
%As it measures the variance term in the risk of \( \tilde{\upsv}_{\GP} \), it might be called the \emph{effective noise level}
%of the problem.
We conclude that the main properties of the pMLE \( \tilde{\upsv}_{\GP} \) 
%including concentration and Fisher and Wilks expansions 
are valid under the condition \( \dimVG \ll n \) meaning sufficiently many observations 
per effective number of parameters.
%, or, equivalently, under sufficient \emph{signal-to-noise ratio}. 

%\Section{Asymptotic normality of the pMLE \( \tilde{\upsv}_{\GP} \)}
%All previous results have been stated for finite samples with explicit error bounds.
%Here we consider a pre-asymptotic setup with a large number of observations \( n \).
%The Fisher expansion \eqref{DGttGtsGDGm13rG} of Theorem~\ref{TFiWititG} states an approximation of the 
%scaled vector \( \DPGP (\tilde{\upsv}_{\GP} - \upsvs_{\GP}) \) by the normalized score \( \DPGP^{-1} \nabla \zeta \).
%%
%Then it is natural to expect that the normalized score \( \DPGP^{-1} \nabla \zeta \) approaches 
%a Gaussian distribution as \( n \) grows.
%We present here a result in a weak topology by considering scalar products 
%\( \bigl\langle \DPGP (\tilde{\upsv}_{\GP} - \upsvs_{\GP}), \uv \bigr\rangle \) for possible directions \( \uv \).
%An extension to other more strong topologies are possible; see e.g. 
%

% !TEX root = ../generic.tex

\Section{The use of \( \DPGPt^{2} \) instead of \( \DPGP^{2} \)}
\label{SDPGPDPGPt}
The penalized information matrix 
\( \DPGP^{2} = \DPGP^{2}(\upsvs_{\GP}) = - \nabla^{2} \E \LGP(\upsvs_{\GP}) \) 
plays an important role in our results.
%By linearity of the stochastic component, it also holds \( \nabla^{2} \E \LGP(\upsvs_{\GP}) 
%= \nabla^{2} \LGP(\upsvs_{\GP}) \).
In particular, \( \DPGP \) describes the shape of the concentration set \( \CA_{\GP} = \upsvs_{\GP} + \UVz_{\GP} \).
%for concentration of \( \tilde{\upsv}_{\GP} \).
However, this matrix is not available as it involves the unknown point \( \upsvs_{\GP} \).
If the matrix function \( \IF(\upsv) \) is locally constant in \( \CA_{\GP} \), one can replace \( \upsvs_{\GP} \) 
with its estimate \( \tilde{\upsv}_{\GP} \).
Variability of \( \IF(\upsv) \), or, equivalently, \( \IF_{\GP}(\upsv) = \IF(\upsv) + \GP^{2} \) 
can be measured 
under the Fr\'echet smoothness of \( f(\upsv) = \E \LGP(\upsv) \) 
by the value \( \dltwbss_{\GP} \) from \eqref{jcxhydtferyufgy7tfdsy7ft}
\( \upsv = \upsvs_{\GP} \), \( \DVL(\upsv) = \DPGP \), and \( \rr = \amax^{-1} \rrGP \).


\begin{proposition}
\label{PDPGPtDPGP}
Assume the conditions of 
%\ifsupnorm{
%Proposition~\ref{PconcMLEgen} or Proposition~\ref{PconcMLEgenc}.
%}{
Proposition~\ref{PconcMLEgenc}
and let \( \dltwbss_{\GP} \leq 1/2 \); see \eqref{jcxhydtferyufgy7tfdsy7ft}.
%} 
The random matrix \( \DPGPt^{2} = \IF_{\GP}(\tilde{\upsv}_{\GP}) \) fulfills on \( \Omega(\xx) \) 
for any \( \uv \in \R^{\dimp} \)
%for an universal constant \( \CONST \)
\begin{EQ}[rcccl]
%    \sup_{\uv \colon \amax \DPGP^{2} \uv \in \UVz} 
    \bigl\| \DPGP^{-1} \DPGPt^{2} \, \DPGP^{-1} - \Id_{\dimp} \bigr\|
    & \leq &
    \dltwbss_{\GP} \, ,
    \qquad
    \bigl\| \DPGP \, \DPGPt^{-2} \, \DPGP - \Id_{\dimp} \bigr\|
    & \leq &
    \frac{\dltwbss_{\GP}}{1 - \dltwbss_{\GP}} \, ,
    \qquad
\label{DPGPm1Cd3rG}
%\end{EQ} 
%and for any \( \uv \in \R^{\dimp} \)
%\begin{EQA}
	\\
	(1 - \dltwbss_{\GP}) \, \| \DPGP \uv \|^{2}
	& \leq &
	\| \DPGPt \uv \|^{2}
	\leq 
	(1 + \dltwbss_{\GP}) \, \| \DPGP \uv \|^{2} .
\label{jamnjhgfrderr5t6784eds}
\end{EQ}
%with \( f(\upsv) = \E \LGP(\upsv) \) 
\end{proposition}

\begin{proof}
The value \( \tilde{\upsv}_{\GP} - \upsvs_{\GP} \) belongs to \( \UVz_{\GP} \) on \( \Omega(\xx) \) and 
\eqref{DPGPm1Cd3rG} follows from \eqref{ghdrd324ee4ew222w3ew}.
\end{proof}


\Section{Smoothness and bias}
\label{Ssmoothbias}
Due to 
%\ifsupnorm{Proposition~\ref{PconcMLEgen} or \ref{PconcMLEgenc}}
{Proposition~\ref{PconcMLEgenc}}, 
the penalized MLE  \( \tilde{\upsv}_{\GP} \) is in fact an estimator of the vector \( \upsvs_{\GP} \).
%In particular, \( \| \DPGP (\tilde{\upsv}_{\GP} - \upsvs_{\GP}) \| \leq \amax^{-1} \rr_{\GP} \)
%with a high probability, where \( \rr_{\GP} = \rr_{\GP}(\xx) \) from \eqref{34rtyghuioiuyhgvftid}
%bounds the norm \( \| \DPGP^{-1} \nabla \zeta \| \).
However, \( \upsvs_{\GP} \) depends on penalization which introduces some bias.
This section discusses whether one can use \( \tilde{\upsv}_{\GP} \) for estimating the underlying truth \( \upsvs \)
defined as the maximizer of the expected log-likelihood:
\( \upsvs = \argmax_{\upsv} \E L(\upsv) \).
%The key argument is the upper bound on the bias \( \biasv_{\GP} = \upsvs_{\GP} - \upsvs \) from 
%Proposition~\ref{Lvarusetb}.
First we describe the bias \( \biasv_{\GP} = \upsvs_{\GP} - \upsvs \) induced by penalization.
%We use that \( \DPGP^{2} = \DP^{2} + \GP^{2} \) with \( \DP^{2} = - \nabla^{2} f(\upsvs_{\GP}) \).
It is important to mention that the previous results about the properties of the pMLE \( \tilde{\upsv}_{\GP} \)
require strong concavity of the expected log-likelihood function \( \E \LGP(\upsv) \) at least in a vicinity 
of the point \( \upsvs_{\GP} \). 
In some sense, this strong concavity is automatically forced 
by the penalizing term in the definition of \( \upsvs_{\GP} \).
However, the underlying truth \( \upsvs = \argmax_{\upsv} \E L(\upsv) \) is the maximizer of the non-penalized 
expected log-likelihood,
and the corresponding Hessian \( \IF(\upsvs) = - \nabla^{2} \E L(\upsvs) \) can degenerate. 
This makes evaluation of the bias more involved.
To bypass this situation, we assume later in this section 
that the Hessian \( \nabla^{2} \E \LGP(\upsv) \) cannot change much in a reasonably large vicinity of \( \upsvs \).
%on the line between \( \upsvs_{\GP} \) and \( \upsvs \). 
This allows to establish an accurate quadratic approximation of \( f(\upsv) \) and to evaluate the bias
\( \biasv_{\GP} = \upsvs_{\GP} - \upsvs \).

Define \( \DPfGP \) by \( \DPfGP^{2} = \IF_{\GP}(\upsvs) \);
cf. \( \DPGP^{2} = \IF_{\GP}(\upsvs_{\GP}) \). 
Let also \( \QP \) be a symmetric matrix satisfying  \( \QP^{2} \leq \DPfGP^{2} \).
Typical examples include \( \QP = \DPGP \), \( \QP = \DPfGP \), and \( \QP^{2} = \nsize \Id_{\dimp} \).
Later we bound the norm \( \| \QP \biasv_{\GP} \| \).
%Introduce a vector
%\begin{EQA}
%	\Av_{\GP} 
%	&=& 
%	- \GP^{2} \upsvs,
%%	\qquad
%%	\av_{\GP} = \QP \, \DPfGP^{-2} \Av_{\GP} = - \QP \, \DPfGP^{-2} \, \GP^{2} \upsvs \, .
%\label{gv8reyuo0hdfyt3hjrfi9}
%\end{EQA}
%and 
Denote %\( \rru = \amax^{-1} \| \av_{\GP} \| = \amax^{-1} \| \QP \, \DPfGP^{-2} \, \GP^{2} \upsvs \| \) 
with \( \amax = 2/3 \)  
\begin{EQ}[rcl]
	\bias_{\GP}
	& \eqdef &
	\| \QP \, \DPfGP^{-2} \, \GP^{2} \upsvs \| ,
	\\
	\dltwbs_{\GP} 
	& \eqdef &
	\sup_{\uv \colon \| \QP \uv \| \leq \amax^{-1} \bias_{\GP}} \,\, 
	\| \DPfGP^{-1} \, \IF_{\GP}(\upsvs + \uv) \, \DPfGP^{-1} - \Id_{\dimp} \| ;
\label{ghdrd324ee4ew222}
\end{EQ}
cf. \eqref{jcxhydtferyufgy7tfdsy7ft} and \eqref{ghdrd324ee4ew222w3ew} for \( f(\upsv) = \E \LGP(\upsv) \).
%Later we present the results on the bias \( \biasv_{\GP} = \upsvs_{\GP} - \upsvs \) under the condition that 
%\( \dltwbs_{\GP} \ll 1 \).
% and this \( \rru \); .
Note that the definition of \( \dltwbss_{\GP} \) in Proposition~\ref{PDPGPtDPGP} uses another \( \rrn = \amax^{-1} \rrGP \),
therefore, different notation.
Proposition~\ref{Pbiasgeneric} yields the following result.

\begin{proposition}
\label{Lvarusetb} 
Let \( \DPfGP^{2} = \IF_{\GP}(\upsvs) \),
%\( \Av_{\GP} = - \GP^{2} \upsvs \),
\( \amax \leq 2/3 \), and \( \bias_{\GP} = \| \QP \, \DPfGP^{-2} \, \GP^{2} \upsvs \| \).
Let also \( \dltwbs_{\GP} \leq 1/3 \); see \eqref{ghdrd324ee4ew222}.
%for \( \fs(\upsv) = \E \LGP(\upsv) \), \( \upsv = \upsvs \), and \( \rr = \rru \), 
Then the bias \( \biasv_{\GP} = \upsvs_{\GP} - \upsvs \) fulfills
%for any linear mapping \( \QP \colon \R^{\dimp} \to \R^{\dimq} \)
\begin{EQA}[rcccl]
	\| \QP \, \biasv_{\GP} \|
	& \leq &
	\frac{\bias_{\GP}}{1 - \dltwbs_{\GP}}  
	&=&
	\frac{1}{1 - \dltwbs_{\GP}} \, \| \QP \, \DPfGP^{-2} \, \GP^{2} \upsvs \|\, ,
\label{11ma3eaelDebQ}
	\\
	\| \QP (\biasv_{\GP} + \DPfGP^{-2} \GP^{2} \upsvs) \|
	& \leq &
	\frac{\dltwbs_{\GP}}{1 - \dltwbs_{\GP}} \, \bias_{\GP}
	&=&
	\frac{\dltwbs_{\GP}}{1 - \dltwbs_{\GP}} \, \| \QP \, \DPfGP^{-2} \, \GP^{2} \upsvs \| .
\label{11ma3eaelDeb}
\end{EQA}
\end{proposition}

%Result \eqref{11ma3eaelDeb} effectively means that \( \biasv_{\GP} \approx \DPfGP^{-2} \Av_{\GP} = (\Id_{\dimp} - \proj_{\GP}) \upsvs \), 
%where the operator \( \Id_{\dimp} - \proj_{\GP} = \DPfGP^{-2} \, \GP^{2} \) is a sub-projector and it can be viewed as 
%an approximation of the projector on the parameter subspace of vectors \( \uv \) with
%\( \| \GP \uv \| \gg \| \DP \uv \| \).
%In this subspace, the penalty term \( \| \GP \uv \| \) dominates and 
%\( \Id_{\dimp} - \proj_{\GP} \) shrinks such \( \uv \) towards zero. 
%The bias term is due to the difference \( \upsvs - \proj_{\GP} \upsvs \approx - \DPfGP^{-2} \, \GP^{2} \upsvs \). 

%Note that under the imposed conditions, the penalized target \( \upsvs_{\GP} \) belongs to local vicinity of \( \upsvs \)
%and by \eqref{ghdrd324ee4ew222w3ew} of Lemma~\ref{LfreTay} 
% \( \DPGP^{2} = \DPGP^{2}(\upsvs_{\GP}) \approx \DPfGP^{2} = \DPGP^{2}(\upsvs) \).

%As special cases of \eqref{11ma3eaelDebQ}, consider \( \QP = \DPfGP \) and \( \QP = \Id_{\dimp} \).
%

\begin{corollary}
\label{CbiasGPb}
Assume the conditions of Proposition~\ref{Lvarusetb}. 
Then 
\begin{EQA}[rcccl]
	\| \DPfGP \, \biasv_{\GP} \|
	& \leq &
	\frac{1}{1 - \dltwbs_{\GP}} \, \| \DPfGP^{-1} \, \GP^{2} \upsvs \| ,
%	\leq 
%	\frac{1}{1 - \dltwbs_{\GP}} \, \| \GP \upsvs \|^{2} \, ,
	\qquad
	\| \biasv_{\GP} \|
	& \leq &
	\frac{1}{1 - \dltwbs_{\GP}} \, \| \DPfGP^{-2} \, \GP^{2} \upsvs \| .
%	\leq 
%	\frac{1}{1 - \dltwbs_{\GP}} \, \| \IF_{\GP}^{-1} \| \, \| \GP \upsvs \|^{2} \, .
\label{0mkvhgjnrw3dfwe3u8gty}
\end{EQA}
The same bounds apply with \( \DPGP^{2} = \IF_{\GP}(\upsvs_{\GP}) \) in place of \( \DPfGP^{2} = \IF_{\GP}(\upsvs) \).
\end{corollary}
This is a special cases of \eqref{11ma3eaelDebQ} with \( \QP = \DPfGP \) and \( \QP = \Id_{\dimp} \).
The last statement is due to Remark~\ref{Rbiasgeneric}.

\Section{Loss and risk of the pMLE}
\label{Slossrisksb}
Now we combine the previous results about the stochastic term \( \tilde{\upsv}_{\GP} - \upsvs_{\GP} \)
and the bias term \( \biasv_{\GP} = \upsvs_{\GP} - \upsvs \) to obtain the sharp bounds 
on the loss and risk of the pMLE \( \tilde{\upsv}_{\GP} \).

%
%In particular, the mentioned ``small bias'' condition means that \( \| \av_{\GP} \| \ll \rr_{\GP} \).
%
%Now we show how the Fisher expansion \eqref{DGttGtsGDGm13rG} enables us to establish sharp finite sample bounds
%for the loss and risk of the estimator \( \tilde{\upsv}_{\GP} \).

\begin{theorem}
\label{PFiWibias}
Assume the conditions of Proposition~\ref{PconcMLEgenc} and \ref{Lvarusetb}.
%Let \( \upsvs \in \Upsd \).
Then on \( \Omega(\xx) \) with \( \P\bigl( \Omega(\xx) \bigr) \geq 1 - 3 \ex^{-\xx} \),
it holds with \( \xiv_{\GP} = \DPGP^{-1} \, \nabla \zeta \), \( \rr_{\GP} \) from \eqref{34rtyghuioiuyhgvftid},
and \( \nsize^{-1} = \| \DPGP^{-2} \| \)
%, and \( \av_{\GP} = \DPGP^{-1} \Av_{\GP} = - \DPGP^{-1} \GP^{2} \upsvs \)
%for the loss \( \bigl\| \QP\bigl( \tilde{\upsv}_{\GP} - \upsvs \bigr) \bigr\| \)
\begin{EQA}[rcccl]
	\| \DPGP \, (\tilde{\upsv}_{\GP} - \upsvs) \|
	& \leq &
	\frac{1 + \sqrt{2 \dltwb_{\GP}}}{1 - \dltwb_{\GP}} \| \xiv_{\GP} \|
%	\rr_{\GP} / (1 - \amax) 
	+ \frac{\| \DPGP^{-1} \GP^{2} \upsvs \|}{1 - \dltwbs_{\GP}}  
	& \leq &
	\frac{1 + \sqrt{2 \dltwb_{\GP}}}{1 - \dltwb_{\GP}} \rr_{\GP}
%	\rr_{\GP} / (1 - \amax) 
	+ \frac{\| \DPGP^{-1} \GP^{2} \upsvs \|}{1 - \dltwbs_{\GP}} \, ,
	\qquad \qquad
\label{rG1r1d3GbvGb}
	\\
	\| \tilde{\upsv}_{\GP} - \upsvs \|
	& \leq &
	\frac{1 + \sqrt{2 \dltwb_{\GP}}}{\sqrt{\nsize} \, (1 - \dltwb_{\GP})} \| \xiv_{\GP} \| 
	+ \frac{\| \DPGP^{-2} \GP^{2} \upsvs \|}{1 - \dltwbs_{\GP}} 
	& \leq &
	\frac{3 \, \rrGP}{\sqrt{\nsize}} + 3 \, \| \DPGP^{-2} \GP^{2} \upsvs \| \, .
\label{g25re9fjfregdndg}
\end{EQA}
\end{theorem}

\begin{proof}
Let \( \Omega(\xx) \) be the random set from \nameref{EU2ref} on which
with \( \| \xiv_{\GP} \| \leq \rrGP \).
It follows from \eqref{DGttGtsGDGm13rG} of Theorem~\ref{TFiWititG} 
%and \( 3 \dltwb_{\GP} \leq \dltwbs_{\GP} \) 
that on \( \Omega(\xx) \) 
with \( \biasv_{\GP} = \upsvs_{\GP} - \upsvs \)
\begin{EQA}
	\bigl\| \DPGP\bigl( \tilde{\upsv}_{\GP} - \upsvs \bigr) + \DPGP \biasv_{\GP} \bigr\|
	& \leq &
	\frac{1 + \sqrt{2 \dltwb_{\GP}}}{1 - \dltwb_{\GP}} \, \bigl\| \xiv_{\GP} \bigr\| \, .
%	+ \dltwbs_{\GP} \| \QP \av_{\GP} \| .
\label{2biGe233GDttGQ}
\end{EQA}
% and \eqref{11ma3eaelDeb} 
This and \eqref{0mkvhgjnrw3dfwe3u8gty} imply \eqref{rG1r1d3GbvGb}.
\end{proof}


%\begin{corollary}
%\label{CPFiWibias}
%Assume the conditions of Proposition~\ref{PconcMLEgenc} and Proposition~\ref{Lvarusetb} with 
%\( \dltwb_{\GP} \leq 1/3 \) and \( \dltwbs_{\GP} \leq 1/3 \).
%With \( \nsize^{-1} = \| \DPGP^{-2} \| \), it holds on \( \Omega(\xx) \)
%\begin{EQA}
%	\| \tilde{\upsv}_{\GP} - \upsvs \|
%	& \leq &
%	\frac{3 \| \xiv_{\GP} \|}{\sqrt{\nsize}} + 3 \| \DPGP^{-2} \GP^{2} \upsvs \| 
%	\leq 
%	\frac{3 \rrGP}{\sqrt{\nsize}} + 3 \| \DPGP^{-2} \GP^{2} \upsvs \| \, .
%\label{g25re9fjfregdndg}
%\end{EQA}
%\end{corollary}

Now we state the results about the risk of the pMLE \( \tilde{\upsv}_{\GP} \).
To avoid technical burden, 
we fix a large \( \xx \), \( \rr_{\GP} = \rr_{\GP}(\xx) \), and exclude an event 
\( \bigl\{ \| \xiv_{\GP} \| > \rr_{\GP} \bigr\} \) 
having an exponentially small probability; see 
condition \eqref{2emxGPm12nz122} of Proposition~\ref{PconcMLEgenc}.
%Remind the definition of the \emph{effective dimension} \( \dimVG = \tr(\DPGP^{-2} \, \VP^{2}) \) from Section~\ref{Scondgeneric}:
%see \nameref{EU2ref}.
%\begin{EQA}
%	\dimVG
%	& \eqdef &
%	\tr(\DPGP^{-2} \, \VP^{2}) .
%\label{fr7fjothnurtujkrt}
%\end{EQA}
%see \eqref{34rtyghuioiuyhgvftid}.
%Below this value will be called the ; cf. \cite{SP2013_rough} and \cite{SpPa2019}.
%Due to the next result,
%it quantifies the variance term in the risk of the pMLE \( \tilde{\upsv}_{\GP} \).

\begin{theorem}
\label{PFiWi2risk}
Assume the conditions of Proposition~\ref{PconcMLEgenc} and Proposition~\ref{Lvarusetb}.
Then for a set \( \Omega(\xx) \) with \( \P\bigl( \Omega(\xx) \bigr) \geq 1 - 3 \ex^{-\xx} \),
it holds with \( \dimVG = \tr(\DPGP^{-2} \, \VP^{2}) \)
\begin{EQA}
	&& \nquad
	\bigl\| \E \, \bigl\{ \DPGP (\tilde{\upsv}_{\GP} - \upsvs) \Ind\bigl( \Omega(\xx) \bigr) \bigr\} \bigr\|
%	&=&
%	\bigl\| \E \QP (\tilde{\upsv}_{\GP} - \upsvs - \DPGP^{-2} \nabla \zeta) \bigr\|
	\leq 
	\frac{1}{1 - \dltwbs_{\GP}} \| \DPGP^{-1} \GP^{2} \upsvs \| 
	+ \frac{\sqrt{3 \dltwb_{\GP}}}{1 - \dltwb_{\GP}} \, \E \| \xiv_{\GP} \| 
	+ \CONSTi_{1} \ex^{-\xx}
	\\
	& \leq &
	\frac{1}{1 - \dltwbs_{\GP}} \| \DPGP^{-1} \GP^{2} \upsvs \| 
	+ \frac{\sqrt{3\dltwb_{\GP}}}{1 - \dltwb_{\GP}} \, \sqrt{\dimVG} 
	+ \CONSTi_{1} \ex^{-\xx} \,\, ,
\label{EtuGus11md3G}
\end{EQA}
and
\begin{EQA}
	&& \nquad
	\E \bigl\{ \| \DPGP \, (\tilde{\upsv}_{\GP} - \upsvs) \|^{2} \Ind\bigl( \Omega(\xx) \bigr) \bigr\}
	\\
	& \leq &
	\left( 1 + \frac{\sqrt{2\dltwb_{\GP}}}{1 - \dltwb_{\GP}} \right)^{2} \, \dimA_{\GP}
%	\\
%	&&
	+ \, \left( \frac{1}{1 - \dltwbs_{\GP}} \| \DPGP^{-1} \GP^{2} \upsvs \| 
		+ \frac{\sqrt{3\dltwb_{\GP}}}{1 - \dltwb_{\GP}} \, \sqrt{\dimVG}  + \CONSTi_{1} \ex^{-\xx} 
	\right)^{2} \, .
%	+ \CONSTi_{2} \ex^{-\xx} 
	\qquad
	\qquad
\label{EQtuGmstrVEQtG}
\end{EQA}
\end{theorem}

\begin{remark}
For \( \dltwbs_{\GP} \), \( \dltwb_{\GP} \)  small, 
\eqref{EQtuGmstrVEQtG} yields classical bias-variance decomposition:
%with \( \av_{\GP} = - \DPGP^{-1} \GP^{2} \upsvs \)
\begin{EQA}
	\E \bigl\{ \| \DPGP \, (\tilde{\upsv}_{\GP} - \upsvs) \|^{2} \Ind\bigl( \Omega(\xx) \bigr) \bigr\}
	& \leq &
	\bigl( \dimVG + \| \DPGP^{-1} \GP^{2} \upsvs \|^{2} \bigr) \bigl\{ 1 + o(1) \bigr\} .
%	\leq 
%	\bigl( \dimVG + \| \GP \upsvs \|^{2} \bigr) \bigl\{ 1 + o(1) \bigr\}.
\label{EQtuGuvus2tr1o1}
\end{EQA}
With \( \nsize^{-1} = \| \DPGP^{-2} \| \), we also obtain
\begin{EQA}
	\E \bigl\{ \nsize \| \tilde{\upsv}_{\GP} - \upsvs \|^{2} \Ind\bigl( \Omega(\xx) \bigr) \bigr\}
	& \leq &
	\bigl( \dimVG + \nsize \| \DPGP^{-2} \GP^{2} \upsvs \|^{2}\bigr) 
	\bigl\{ 1 + o(1) \bigr\} .
%	\leq 
%	\bigl( \dimVG + \| \GP \upsvs \|^{2} \bigr) \bigl\{ 1 + o(1) \bigr\}.
\label{EQtuGuvus2tr1o1n}
\end{EQA}
Moreover, under the small bias condition \( \| \DPGP^{-2} \GP^{2} \upsvs \|^{2} \ll \dimA_{\GP}/\nsize \), 
the impact of the bias induced by penalization is negligible. 
The relation \( \| \DPGP^{-2} \GP^{2} \upsvs \|^{2} \asymp \dimA_{\GP}/\nsize \) is usually referred to as ``bias-variance trade-off''.
Our bound is sharp in the sense that even for the special case of a linear models, 
\eqref{EQtuGuvus2tr1o1} becomes equality.
\end{remark}
%

\begin{proof}
Below we denote \( \Ex \eta = \E \bigl\{ \eta \Ind\bigl( \Omega(\xx) \bigr) \bigr\} \) for any r.v. \( \eta \).
As \( \E \xiv_{\GP} = 0 \), we derive 
\begin{EQA}
	\Ex \bigl\{ \DPGP (\tilde{\upsv}_{\GP} - \upsvs) \bigr\}
	&=&
	\Ex \DPGP (\tilde{\upsv}_{\GP} - \upsvs - \xiv_{\GP}) 
	- \E \xiv_{\GP} \Ind\bigl( \Omega^{c}(\xx) \bigr) .
\label{EQtuGusIOQPc}
\end{EQA}
For the first term we apply \eqref{DGttGtsGDGm13rG} and \eqref{0mkvhgjnrw3dfwe3u8gty} yielding
\begin{EQA}
	\| \Ex \DPGP (\tilde{\upsv}_{\GP} - \upsvs - \xiv_{\GP}) \|
	& \leq &
	\frac{\| \DPGP^{-1} \GP^{2} \upsvs \| }{1 - \dltwbs_{\GP}} + \frac{\sqrt{3 \dltwb_{\GP} \, \dimVG}}{1 - \dltwb_{\GP}} \, .
\label{7554gtnhbgu8bg87yftwe}
\end{EQA}
To show \eqref{EtuGus11md3G}, we also have to bound the tail moments of 
\( \| \xiv_{\GP} \| \):
\begin{EQA}
	\bigl\| \E \xiv_{\GP} \Ind\bigl( \Omega^{c}(\xx) \bigr) \bigr\|
	& \leq &
	\E \| \xiv_{\GP} \| \Ind\bigl( \Omega^{c}(\xx) \bigr) 
	\leq 
	\ex^{-\xx/2}.
\label{exmxm2E12x2}
\end{EQA}
This can be easily done using deviation bounds for the quadratic form \( \| \xiv_{\GP} \|^{2} \);
see Theorem~\ref{Tdevboundinf}.
Similarly one can bound the variance of \( \DPGP \, \tilde{\upsv}_{\GP} \).
With \( \BB_{\GP} = \DPGP^{-1} \VP^{2} \DPGP^{-1} \)
\begin{EQA}
	\Var_{\xx} \bigl( \DPGP \, \tilde{\upsv}_{\GP} \bigr)
	& \leq &
	\Ex \,\bigl\{ \DPGP \, (\tilde{\upsv}_{\GP} - \upsvs_{\GP}) \bigr\} 
	\bigl\{ \DPGP \, (\tilde{\upsv}_{\GP} - \upsvs_{\GP}) \bigr\}^{\T} 
	\\
	& \leq &
	\left( 1 + \frac{\sqrt{2\dltwb_{\GP}}}{1 - \dltwb_{\GP}} \right)^{2} 
		\E \bigl( \xiv_{\GP} \, \xiv_{\GP}^{\T} \bigr)
	= 
	\left( 1 + \frac{\sqrt{2\dltwb_{\GP}}}{1 - \dltwb_{\GP}} \right)^{2} \BB_{\GP} \, .
\label{VaQtuGd3G1md3Gr2}
\end{EQA}
This yields for the quadratic risk \( \E \| \DPGP \, (\tilde{\upsv}_{\GP} - \upsvs) \|^{2} \)
\begin{EQA}
	\Ex \, \| \DPGP \, (\tilde{\upsv}_{\GP} - \upsvs) \|^{2} 
	& \leq &
	\tr \Var_{\xx}\bigl\{ \DPGP \, (\tilde{\upsv}_{\GP} - \upsvs) \bigr\}
	+ \bigl\| \Ex \, \DPGP (\tilde{\upsv}_{\GP} - \upsvs) \bigr\|^{2}
\label{EQtuGmstrVEQtGp}
\end{EQA}
and \eqref{EQtuGmstrVEQtG} follows. 
\end{proof}



%Finally we state the Wilks expansion for the quantity \( 2 \LGP(\tilde{\upsv}_{\GP}) - 2 \LGP(\upsvs) \) 
%and specify it under the small bias condition \( \| \av_{\GP} \| \ll \rr_{\GP} \).
%
%
%\begin{proposition}
%\label{PsqWilks}
%It holds under the conditions of Proposition~\ref{PconcMLEgenc} on the set \( \Omega(\xx) \)
%\begin{EQA}
%	\Bigl| \sqrt{2 \LGP(\tilde{\upsv}_{\GP}) - 2 \LGP(\upsvs)}
%		- \bigl\| \DPGP^{-1} \nabla \zeta + \DPGP \biasv_{\GP} \bigr\|
%	\Bigr|
%	& \leq &
%	2 \sqrt{3\dltwb_{\GP}} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\| 
%	+ \frac{\dltwb_{\GP}}{2 (1 - \dltwbs_{\GP})} \| \av_{\GP} \| \, ,
%\label{222bb23G2L2rG}
%	\\
%	\Bigl| \sqrt{2 \LGP(\tilde{\upsv}_{\GP}) - 2 \LGP(\upsvs)}
%		- \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|
%	\Bigr|
%	& \leq &
%	2 \sqrt{3\dltwb_{\GP}} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\| 
%	+ \frac{1 + \dltwb_{\GP}/2}{1 - \dltwbs_{\GP}} \, \| \av_{\GP} \| \, .
%\label{222bb23G2L2rG}
%\end{EQA}
%\end{proposition}
%
%\begin{proof}
%By \eqref{3d3Af12DGttG} of Theorem~\ref{TFiWititG} 
%\begin{EQA}
%	2 \LGP(\tilde{\upsv}_{\GP}) - 2 \LGP(\upsvs)
%	& \leq &
%	(1 + \dltwb_{\GP}) \bigl\| \DPGP (\tilde{\upsv}_{\GP} - \upsvs) \bigr\|^{2} \, .
%\label{1p3a3GDm1ntz}
%\end{EQA}
%Moreover, \eqref{DGttGtsGDGm13rG} ensures that
%\begin{EQA}
%%	&& \nquad
%	\sqrt{2 \LGP(\tilde{\upsv}_{\GP}) - 2 \LGP(\upsvs)}
%%	\\
%	& \leq &
%	\sqrt{1 + \dltwb_{\GP}} \Bigl( \bigl\|\DPGP^{-1} \nabla \zeta + \DPGP \biasv_{\GP} \bigr\|
%	+ \frac{\sqrt{3\dltwb_{\GP}}}{1 - \dltwb_{\GP}} \, \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|
%	\Bigr)
%\label{sq2LGtG2s2}
%\end{EQA}
%yielding by \eqref{11ma3eaelDeb}
%\begin{EQA}
%	&& \nquad
%	\sqrt{2 \LGP(\tilde{\upsv}_{\GP}) - 2 \LGP(\upsvs)}
%		- \bigl\| \DPGP^{-1} \nabla \zeta + \DPGP \biasv_{\GP} \bigr\|
%	\\
%	& \leq &
%	\frac{\dltwb_{\GP}}{2}\bigl\| \DPGP^{-1} \nabla \zeta + \DPGP \biasv_{\GP} \bigr\|
%	+ \frac{\sqrt{\dltwa_{\GP} (1 + \dltwb_{\GP})}}{1 - \dltwb_{\GP}} \, \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|
%	\\
%	& \leq &
%	2 \sqrt{3\dltwb_{\GP}} \bigl\| \DPGP^{-1} \nabla \zeta \bigr\|
%	+ \frac{\dltwb_{\GP}}{2(1 - \dltwbs_{\GP})} \| \av_{\GP} \| .
%\label{bG2d3G2sd3Gs2}
%\end{EQA}
%The inverse inequality and the  second statement can be proved in a similar way.
%\end{proof}
%




==> smoothpen.tex <==
% !TEX root = ../generic.tex
\Chapter{Smooth priors and rate over Sobolev classes}
\label{Spriorexample}
This section presents some examples of choosing \( \GP^{2} \) for 
achieving the ``bias-variance trade-off''
and obtaining rate optimal results.
Define the background true parameter
\begin{EQA}
	\upsvs 
	&=& 
	\argmax_{\upsv} \E L(\upsv) .
\label{v43hrf5fjh9ehft6f}
\end{EQA}
Remind the notation \( \LGP(\upsv) \eqdef L(\upsv) - \| \GP \upsv \|^{2}/2 \),
\begin{EQA}[rcccl]
	\tilde{\upsv}_{\GP}
	& \eqdef &
	\argmax_{\upsv \in \Ups} \LGP(\upsv)
\label{v8j3gug5ejfgifkri}
	\qquad	
	\upsvs_{\GP}
	& \eqdef &
	\argmax_{\upsv \in \Ups} \E \LGP(\upsv) .
\label{upssaruELuaiUa}
\end{EQA}
Also, for any \( \upsv \in \Ups \),
\begin{EQA}[rcccl]
	\IF(\upsv) 
	&=& 
	- \nabla^{2} \E L(\upsv) ,
	\qquad
	\IF_{\GP}(\upsv) 
	&=& 
	- \nabla^{2} \E \LGP(\upsv) 
	= 
	\IF(\upsv) + \GP^{2} .
\label{e456yhgfr567uhgfa}
\end{EQA}
Posterior concentration relies on the \emph{Laplace effective dimension}
\begin{EQA}
	\dimA(\upsv)
	& \eqdef &
	\tr\bigl\{ \IF_{\GP}^{-1}(\upsv) \, \IF(\upsv) \bigr\} 
\label{0n2ig82jfirjqgdkgyehj}
\end{EQA}
for \( \upsv \) in a small vicinity \( \CA_{\GP} \).
The pMLE \( \tilde{\upsv}_{\GP} \) concentrates in a vicinity of \( \upsvs_{\GP} \)
and the concentration radius is described via the \emph{effective dimension}
\begin{EQA}
	\dimG
	& \eqdef &
	\tr\bigl( \IF_{\GP}^{-1} \VP^{2} \bigr) ,
\label{ufh3u3whdjhduwkfig2}
\end{EQA}
where for \( \IF_{\GP} = \IF_{\GP}(\upsvs_{\GP}) \) and \( \VP^{2} = \Var (\nabla \zeta ) \).
It is worth noting that under conditions of Proposition~\ref{Lvarusetb} 
\( \IF_{\GP}(\upsvs) \) can be used in place of \( \IF_{\GP} \).
Moreover,
\( \VP^{2} = \IF(\upsvs) \) under the correct model specification.

Theorem~\ref{PFiWi2risk} yields the following bound for the risk of \( \tilde{\upsv}_{\GP} \): %with \( \nsize^{-1} = \| \DPGP^{-2} \| \)
\begin{EQA}
	\E \| \DPGP (\tilde{\upsv}_{\GP} - \upsvs) \|^{2}
	& \lesssim &
	\dimG + \| \DP_{\GP}^{-1} \GP^{2} \upsvs \|^{2} \, .
\label{bnjmb3ed6w2jh21fg7fj}
\end{EQA}
This suggest to select the operator \( \GP^{2} \) which ensures the ``bias-variance trade-off'' 
\( \| \DP_{\GP}^{-1} \GP^{2} \upsvs \|^{2} \asymp \dimG \).

\Section{Bias-variance trade-off under \( \GPa \)-smoothness}
\label{SGPasmooth}
Suppose that \( \upsvs \) is \( \GPa \)-smooth, that is,
for a given matrix \( \GPa^{2} \)
\begin{EQA}
	\| \GPa \upsvs \|^{2}
	& \leq &
	1 .
\label{d4hgergv76ehrfrtfge}
\end{EQA}
Consider the univariate family of penalizing/precision matrices \( \GP^{2} \) of the form \( \GP^{2} = \CGP \GPa^{2} \).
Later we discuss a choice of the value \( \CGP \) ensuring the bias-variance relation 
\( \| \DP_{\GP}^{-1} \GP^{2} \upsvs \|^{2} \asymp \dimG \).
Note first that
\begin{EQA}
	\| \DP_{\GP}^{-1} \GP^{2} \upsvs \|^{2}
	& \leq &
	\| \GP \upsvs \|^{2} =	\CGP \, \| \GPa \upsvs \|^{2} 
	= 
	\CGP .
\label{6kv9gvbjdfcvw2cdged8e}
\end{EQA}
%
Next we consider the variance term measured by the effective dimension \( \dimG \).
Under the conditions of Proposition~\ref{Lvarusetb} and correct model specification, 
we may slightly change the definition to
\begin{EQA}
	\dimG
	&=&
	\dimA(\CGP)
	=
	\tr (\DPf^{2} \, \DPfGP^{-2})
	=
	\tr\bigl\{ \DPf^{2} (\DPf^{2} + \CGP \GPa^{2})^{-1} \bigr\} ,
\label{u98gfw3wd7uewj4ert7yg}
\end{EQA}
where \( \DPf^{2} = \IF(\upsvs) \).
The definition is particularly transparent for \( \DPf^{2} = \nsize \Id_{\dimp} \):
\begin{EQA}
	\dimA(\CGP)
	&=&
	\tr\bigl( \Id_{\dimp} + \nsize^{-1} \CGP \, \GPa^{2} \bigr)^{-1} .
\label{c78ju43njvf6vf4e3tg9ythgh}
\end{EQA}
Define also 
\begin{EQA}
	\rr(\CGP)
	&=&
	\sqrt{\dimA(\CGP)} + \sqrt{2 \xx} .
\label{3gyvf76gv7r4ur45r56}
\end{EQA}
Theorem~\ref{PFiWibias}, \eqref{rG1r1d3GbvGb}, yields the following bound.

\begin{theorem}
\label{LbiasCGPw}
Assume \( \| \GPa \upsvs \| \leq 1 \).
Consider \( \GP^{2} = \CGP \, \GPa^{2} \), \( \DPfGP^{2} = \DPf^{2} + \CGP \GPa^{2} \).
Suppose the conditions of Proposition~\ref{PconcMLEgenc} and \ref{Lvarusetb} hold for this choice of \( \GP^{2} \).
Then on \( \Omega(\xx) \), the estimate \( \tilde{\upsv}_{\GP} \) fulfills 
for some fixed constant \( \CONST \)
\begin{EQA}
	\| \DPfGP (\tilde{\upsv}_{\GP} - \upsvs) \|
	& \leq &
	2 \rr(\CGP) + 	\amax^{-1} \CGP^{1/2} \, .
\label{0mkvhgjnrw3dfwe3u8CGPw}
\end{EQA}
\end{theorem}

Clearly \( \dimA(0) = \dimp \) and \( \dimA(\CGP) \) monotonously decreases to zero as \( \CGP \) grows to infinity
provided that \( \GPa^{2} \) is positive definite.
Therefore, for any fixed \( \CONSTbal \), the equation
\begin{EQA}
	\rr(\CGP)
	&=&
	\CONSTbal \, \CGP^{1/2}
\label{h0hit5ti85tjrtfg78}
\end{EQA}
has a unique solution \( \CGP = \CGPs \) leading to the desired ``bias-variance trade-off''. 

\begin{theorem}
\label{LbiasCGP}
Assume \( \| \GPa \upsvs \| \leq 1 \).
With a fixed \( \CONSTbal \), define \( \CGPs \) by \( \dimA(\CGPs) = \CONSTbal \, \CGPs \); see \eqref{u98gfw3wd7uewj4ert7yg}.
Define also \( \GP_{\CGPs}^{2} = \CGPs \, \GPa^{2} \), \( \DPf_{\CGPs}^{2} = \DPf^{2} + \CGPs \GPa^{2} \).
Suppose the conditions of Proposition~\ref{PconcMLEgenc} and \ref{Lvarusetb} hold for this choice of \( \GP^{2} = \GP_{\CGPs}^{2} \).
Then on \( \Omega(\xx) \), the estimate \( \tilde{\upsv}_{\CGPs} = \tilde{\upsv}_{\GP_{\CGPs}} \) fulfills 
for some fixed constant \( \CONST \)
\begin{EQA}
	\| \DPf_{\CGPs} (\tilde{\upsv}_{\CGPs} - \upsvs) \|
	& \leq &
	\CONST \CGPs^{1/2} \, .
\label{0mkvhgjnrw3dfwe3u8CGP}
\end{EQA}
With \( \DPf^{2} = \nsize \Id_{\dimp} \), this implies
\begin{EQA}
	\| \tilde{\upsv}_{\CGPs} - \upsvs \|^{2}
	& \leq &
	{\CONST \CGPs}/{\nsize} \, .
\label{0mkvhgjnrw3dfwe3u8CGPn}
\end{EQA}
\end{theorem}


\begin{remark}
The value \( \dimA(\CGP) \) from \eqref{u98gfw3wd7uewj4ert7yg} can be written as
\begin{EQA}
	\dimA(\CGP)
	&=&
	\tr (\Id_{\dimp} + \CGP \DPf^{-1} \, \GPa^{2} \, \DPf^{-1})^{-1} .
\label{78cvhufu7yejhedukfiuer}
\end{EQA}
The operator \( \proj(\CGP) = (\Id_{\dimp} + \CGP \DPf^{-1} \, \GPa^{2} \, \DPf^{-1})^{-1} \) is obviously
a sub-projector in \( \R^{\dimp} \).
In many situation, its trace can be well approximated by the dimension of the subspace in \( \R^{\dimp} \)
on which \( \CGP \DPf^{-1} \, \GPa^{2} \, \DPf^{-1} \leq \Id_{\dimp} \); see the example later for the case 
of Sobolev smoothness.
In particular, with \( \DPf^{2} = \nsize \Id_{\dimp} \), the corresponding subspace is spanned by the eigenvectors
of \( \GPa^{2} \) with eigenvalues \( \gp_{j}^{2} \leq n/\CGP \).
\end{remark}

The obtained bound can be extended to the case 
when the smoothness of \( \upsvs \) is measured using a different operator \( \GPa \) than \( \GP \).
An important example corresponds to a \( (\smp,\CGP) \)-smooth prior 
and a signal \( \upsvs \) is from a Sobolev ball with the smoothness degree \( \smpa \neq \smp \);
see Section~\ref{Ssmoothprior}.
%\ifapp{Section~\ref{Ssmoothprior}}{Section~\ref{SGBvM}}.
Suppose \( \upsvs \) is \( \GPa \)-smooth, and \( \CGPs \) is the corresponding solution of \eqref{h0hit5ti85tjrtfg78}
leading to \( \GP_{\CGPs}^{2} = \CGPs \, \GPa^{2} \) and \( \DPf_{\CGPs}^{2} = \DPf^{2} + \CGPs \GPa^{2} \).
We now consider some other penalizing matrix \( \GP^{2} \).


\begin{theorem}
\label{Pbiassmoone}
Let \( \upsvs \) follow \eqref{d4hgergv76ehrfrtfge} and \( \CGPs \) solve \eqref{h0hit5ti85tjrtfg78}.
Fix \( \GP_{\CGPs}^{2} = \CGPs \, \GPa^{2} \) and \( \DPf_{\CGPs}^{2} = \DPf^{2} + \CGPs \GPa^{2} \).
Suppose for some other \( \GP^{2} \), it holds
\begin{EQA}
	\DPf_{\GP}^{-2} \GP^{2}
	& \leq &
	\CONSTGP \, \DPf_{\CGPs}^{-2} \, \GP_{\CGPs}^{2}
\label{hgjkjhyoie3r56dftrtyf}
\end{EQA}
with a fixed constant \( \CONSTGP \),
and the conditions of Proposition~\ref{PconcMLEgenc} and \ref{Lvarusetb} hold for this choice of \( \GP^{2} \).
Then on \( \Omega(\xx) \) with 
\( \nsize^{-1} = \| \DPfGP^{-2} \| \vee \| \DPf_{\CGPs}^{-2} \| \)
\begin{EQA}[rcl]
	\sqrt{\nsize} \| \tilde{\upsv}_{\GP} - \upsvs \|
	& \leq &
	\CONST \, \CONSTGP \, \CGPs^{1/2} \, .
\label{vfgd32hvfbdgi8ghj89ne}
\end{EQA}
\end{theorem}

\begin{proof}
Apply \eqref{g25re9fjfregdndg} and \eqref{hgjkjhyoie3r56dftrtyf}.
%See \eqref{11ma3eaelDebQbgen} of Proposition~\ref{Pbiasgeneric}.
\end{proof}

Some sufficient conditions for \eqref{hgjkjhyoie3r56dftrtyf} are given in Lemma~\ref{Lsmoothbiase}.


\Section{Smooth penalty and rate of estimation over Sobolev balls}
\label{SrateSobball}
This section illustrates the general results for the case of a smooth penalty \( \GP^{2} \)
for a smooth signal \( \upsvs \) in a Sobolev sense.
Our main intension is to demonstrate that the obtained finite sample bounds imply the well known results on the rate of estimation
under standard smoothness assumptions.
We follow the setup of Section~\ref{Spriors} and assume the diagonal structure of the penalizing matrix 
\( \GP^{2} = \diag(\gp_{1}^{2},\ldots,\gp_{\dimp}^{2}) \) with eigenvalues
\( \gp_{j}^{2} \) satisfying the condition of polynomial growth \eqref{sumjJgjm2C}.
We also assume that the information matrix \( \IF = \IF(\upsvs) \) satisfies \eqref{uVmGu2C1C2gen}:
\begin{EQ}[rcccl]
	\CONSTIF^{-1} \, \nsize \| \uv \|^{2} 
	& \leq &
	\bigl\langle \IF \uv, \uv \bigr\rangle
	& \leq &
	\CONSTIF \, \nsize \| \uv \|^{2},
	\qquad
	\uv \in \R^{\dimp} \, .
\label{uVmGu2C1C2genS}
\end{EQ}
with \( \nsize \) meaning the sample size, 
while \( \VP^{2} \) satisfies \eqref{uVmGu2C1C2genV}:
\begin{EQ}[rcccl]
	\CONSTV^{-1} \, \| \IF \uv \|^{2} 
	& \leq &
	\| \VP \uv \|^{2}
	& \leq &
	\CONSTV \, \| \IF \uv \|^{2},
	\qquad
	\uv \in \R^{\dimp} \, .
\label{uVmGu2C1C2genVS}
\end{EQ}
%Here \( \nsize \) means a sample size; see, e.g., Section~\ref{SGBvM}.


%\Subsection{Roughness penalty and rate of estimation over Sobolev balls}
%\label{SsobolevGLM}
%
%Regarding the effective dimension term \( \dimG \), Section~\ref{Ssmoothprior} provides some 
%natural conditions on penalty matrix \( \GP^{2} \) allowing some rather precise bounds.

\medskip
To illustrate the obtained results, assume that \( \upsvs \) belongs to a Sobolev ball \( \BBB(\smpa,\CGPa) \):
\begin{EQA}
	\BBB(\smpa,\CGPa)
	& \eqdef &
	\Bigl\{ \upsv = (\ups_{j}) \colon \sum_{j \geq 1} j^{2\smpa} \ups_{j}^{2} \leq \CGPa \Bigr\} 
\label{BBBsttsjj1sj2}
\end{EQA}
with \( \smpa > 0 \) and \( \CGPa \asymp 1 \); see Section~\ref{Ssmoothprior}.
First we discuss a smoothness-aware choice of \( \GP^{2} = \diag(\gp_{1}^{2},\ldots,\gp_{\dimp}^{2}) \) assuming \( \smpa > 1/2 \) known.
By \( \CONST \) we denote some fixed constant possibly depending on the other constants in our conditions like
\( \CONSTIF \), \( \CONSTV \), \( \smpa \), \( \hmax_{3} \), \( \CONSTGP \).

\begin{theorem}
\label{CGLMlossGP}
%Assume 
%\nameref{Eref},
%\nameref{EU2ref},
%\nameref{LLref},
%\nameref{LLtS3ref}.
Let also \eqref{uVmGu2C1C2genS} and \eqref{uVmGu2C1C2genVS} hold
and \( \upsvs \in \BBB(\smpa,\CGPa) \), \( \smpa > 1/2 \).
%
Define \( \GP^{2} = \diag(\gp_{1}^{2},\ldots,\gp_{\dimp}^{2}) \) with
\( \gp_{j}^{2} = \CGP \, \CGPa^{-1} j^{2\smpa} \)
for \( \CGP \geq \CONST \CGPa \, \nsize^{1 - 2 \smpa} \).
Suppose the conditions of Proposition~\ref{PconcMLEgenc} and \ref{Lvarusetb} hold for this choice of \( \GP^{2} \).
Then on \( \Omega(\xx) \)
\begin{EQA}
	\| \DPGP (\tilde{\upsv}_{\GP} - \upsvs) \|^{2}
	& \lesssim &
	( \CGP^{-1} \CGPa \, \nsize)^{1/(2\smpa)} + \CGP .
\label{bnjhuy0w9e8r7t6bcgvftr}
\end{EQA}
Furthermore, the choice 
\begin{EQA}
	\CGP 
	&=& 
	(\CGPa \nsize)^{1/(2\smpa+1)} \eqdef \mmps
\label{kvytft64cdfrtdr213ere}
\end{EQA} 
leads to
\begin{EQA}
	\GP^{2} 
	&=& 
	\mmps \, \CGPa^{-1} \diag\{ j^{2\smpa} \}_{j\geq 1} 
	=
	\CGPa^{- 2\smpa/(2\smpa+1)} \, \nsize^{1/(2\smpa+1)} \diag\{ j^{2\smpa} \}_{j\geq 1} 
\label{njbdfhedue437dfhgv6te}
\end{EQA}
and yields for \( \nsize \geq \CONSTn \)
\begin{EQ}[rcl]
	\| \DPGP (\tilde{\upsv}_{\GP} - \upsvs) \|^{2}
	& \lesssim &
	\mmps
	=
	(\CGPa \nsize)^{1/(2\smpa+1)} \, ,
	\\
	\| \tilde{\upsv}_{\GP} - \upsvs \|^{2}
	& \lesssim &
	\mmps \, n^{-1}
	=
	\CGPa^{1/(2\smpa+1)} \, \nsize^{-2\smpa/(2 \smpa + 1)} .
\label{bnjhuy0w9e8r7t6bcgvftrop}
\end{EQ}
\end{theorem}

\begin{proof}
Define \( \mm \) by the relation \( \gp_{\mm}^{2} \approx n \).
This leads to \( \mm \approx (\CGP^{-1} \CGPa \, \nsize)^{1/(2\smpa)} \). 
By Lemma~\ref{LeffdimG} \( \dimG \asymp \mm \).
The condition \( \CGP \geq \CONST \CGPa \, \nsize^{1 - 2 \smpa} \) with a properly selected \( \CONST \)
ensures \( \dimG \ll \nsize \) and hence, \( \rrGP \, n^{-1/2} \) is sufficiently small.
This enables us to apply Proposition~\ref{PconcMLEgenc} and Theorem~\ref{TFiWititG}.  
Furthermore, smoothness of \( \upsvs \in \BBB(\smpa,\CGPa) \) and the definition of 
\( \GP^{2} = \CGP \, \CGPa^{-1} \diag\{ j^{2\smpa} \}_{j\geq 1} \) imply \( \| \GP \upsvs \|^{2} \leq \CGP \)
and hence, \( \| \DP_{\GP}^{-1} \GP^{2} \upsvs \|^{2} \leq \CGP \).
This and \eqref{EQtuGuvus2tr1o1} prove \eqref{bnjhuy0w9e8r7t6bcgvftr}.
Optimizing its right hand-side w.r.t. \( \CGP \) leads to the \( \CGP \asymp \mmps = (\CGPa \nsize)^{1/(2\smpa+1)} \).
The condition \( \mmps \ll \nsize \) reads \( \nsize^{2\smpa} \geq \CONST \CGPa \) and it is automatically fulfilled 
for \( \nsize \) sufficiently large.
%and 
%\begin{EQA}
%	\mmps
%	& \approx &
%	\CGP = (\CGPa \nsize)^{1/(2\smpa+1)} \, .
%\label{cnmvytjhih85jheyewewe}
%\end{EQA}
This yields the final result \eqref{bnjhuy0w9e8r7t6bcgvftrop}.
\end{proof}

With \( \CGPa \asymp 1 \), this result yields the optimal rate of estimation 
\( \| \tilde{\upsv}_{\GP} - \upsvs \|^{2} \lesssim\nsize^{-2\smpa/(2 \smpa + 1)} \) 
over the smoothness class \( \BBB(\smpa,\CGPa) \) from \eqref{BBBsttsjj1sj2}
for the pMLE \( \tilde{\upsv}_{\GP} \) with \( \GP^{2} \) from \eqref{njbdfhedue437dfhgv6te}.

Further we check the situation when \( \upsvs \in \BBB(\smpa,\CGPa) \) but 
we use \( \GP^{2} = \CGP^{-1} \diag\{ j^{2\smp} \}_{j\geq 1} \) for \( \smp \neq \smpa \).
The main question is a proper choice of the scaling factor \( \CGP \) to ensure the same in order accuracy as 
for the \( \smpa \)-aware choice.
%
Lemma~\ref{LeffdimG} provides the key argument: the index \( \mmps \) from \eqref{kvytft64cdfrtdr213ere} should be preserved.
Due to Lemma~\ref{Lsmoothbiase}, to make the construction rigorous we also need to ensure \( \smp \geq \smpa \).
This can be achieved by selecting a reasonably large \( \smp \), e.g. \( \smp = 4 \) or \( \smp = 5 \).
Now the approach can be summarized as follows. 
Under the assumption \( \upsvs \in \BBB(\smpa,\CGPa) \) and \( n^{-1} \asymp \| \DP^{-2} \| \),
we fix \( \mmps \) by \eqref{kvytft64cdfrtdr213ere}.
With \( \GP^{2} = \CGP^{-1} \diag\{ j^{2\smp} \} \), the index \( \mm \) corresponding to \( \gp_{\mm}^{2} \approx \nsize \)
is given by \( \mm \approx (\CGP \, \nsize)^{1/(2\smp)} \).
This leads to the relation
\begin{EQA}
	(\CGP \, \nsize)^{1/(2\smp)}
	& \approx &
	\mmps
	=
	(\CGPa \nsize)^{1/(2\smpa+1)}
\label{6drvjhggv74e3ujf6hgewt}
\end{EQA}
and to the solution 
\begin{EQA}
	\CGP
	& \approx &
	\nsize^{-1} \mmps^{2\smp}
	=
	\nsize^{-1} (\CGPa \nsize)^{2\smp/(2\smpa+1)} .
\label{nmgvctf5rtrtdw2gf56} 
\end{EQA}
Alternatively one can apply the \( \mmps \)-truncation prior with \( \mmps \) from \eqref{6drvjhggv74e3ujf6hgewt}.
The next result assumes again \( \upsvs \in \BBB(\smpa,\CGPa) \) but for any \( \smpa > 0 \).

\begin{theorem}
\label{PGLMlossGPg}
%Assume 
%\nameref{Eref},
%\nameref{EU2ref},
%\nameref{LLref},
%\nameref{LLtS3ref},
%\eqref{uVmGu2C1C2genS}, and \eqref{uVmGu2C1C2genVS}.
Let also \( \upsvs \in \BBB(\smpa,\CGPa) \), \( \smpa > 0 \).
Define %\( \mms = (\CGPa \nsize)^{1/(2\smpa+1)} \) and 
\( \GP^{2} = \CGP^{-1} \diag\{ j^{2\smp} \}_{j\geq 1} \) for some \( \smp > 1/2 \), \( \smp \geq \smpa \),
and \( \CGP \) from \eqref{6drvjhggv74e3ujf6hgewt} or \eqref{nmgvctf5rtrtdw2gf56}.
Suppose the conditions of Proposition~\ref{PconcMLEgenc} and \ref{Lvarusetb} hold for this choice of \( \GP^{2} \).
Then bounds \eqref{bnjhuy0w9e8r7t6bcgvftrop} continue to hold on \( \Omega(\xx) \) provided \( \nsize \geq \CONSTn \).
\end{theorem}

\begin{proof}
Lemma~\ref{LeffdimG} yields \( \dimG \asymp (\CGP \nsize)^{1/(2\smp)} \asymp \mmps \).
Further, Lemma~\ref{Lsmoothbiase} ensures condition \eqref{hgjkjhyoie3r56dftrtyf} of Proposition~\ref{Pbiassmoone}
\( \DPGP^{-2} \GP^{2} \leq \CONSTGP \DP_{\GPa}^{-2} \GPa^{2} \) for a constant \( \CONSTGP \) depending on \( \smpa \) and \( \smp \) only.
The result follows now similarly to \eqref{bnjhuy0w9e8r7t6bcgvftrop}.
\end{proof}


\ifapp{
\Section{Bayesian inference under Sobolev smoothness}
Here we continue the discussion of Section~\ref{SrateSobball} assuming \( \upsvs \in \BBB(\smpa,\CGPa) \) with 
\( \CGPa \asymp 1 \).
A rate-optimal choice of the prior covariance \( \GP^{2} \) is an issue to address.
%We follow Section~\ref{SrateSobball} which focuses on mimicking the proper effective dimension. 
%Under \eqref{uVmGu2C1C2genS}, define \( \GP^{2} = \CGP^{-1} \diag\{ j^{2\smp} \}_{j\geq 1} \) 
%for some \( \smp > 1/2 \), \( \smp \geq \smpa \), 
%and \( \CGP \) from \eqref{6drvjhggv74e3ujf6hgewt} or \eqref{nmgvctf5rtrtdw2gf56}.

\begin{theorem}
\label{TLaplaceGP}
Assume \nameref{Eref},
\nameref{EU2ref},
\nameref{LLCref}, \nameref{LLtS3ref}.
Let also \eqref{uVmGu2C1C2genS} hold
and \( \upsvs \in \BBB(\smpa,\CGPa) \), \( \smpa > 0 \).
Define %\( \mms = (\CGPa \nsize)^{1/(2\smpa+1)} \) and 
\( \GP^{2} = \CGP^{-1} \diag\{ j^{2\smp} \}_{j\geq 1} \) for \( \smp > 1/2 \), \( \smp \geq \smpa \),
and \( \CGP \) from \eqref{6drvjhggv74e3ujf6hgewt} or \eqref{nmgvctf5rtrtdw2gf56}.
Then %the concentration bound \eqref{poybf3679jd532ff2st} holds
for \( \nsize \geq \CONSTn \), it holds on \( \Omega(\xx) \)
\begin{EQA}
	\P\Bigl( \| \vupsv_{\GP} - \tilde{\upsv}_{\GP} \| > \CONST \nsize^{-\smpa/(2\smpa+1)} \Cond \Yv \Bigr)
	& \leq &
	\ex^{-\xx} .
\label{0j7jds2fc56gh98hbt3w}
\end{EQA}
Moreover, if \( \smpa > 1 \), then 
%the Laplace approximation results \eqref{scdugfdwyd2wywy26e6de432} continue to hold 
on \( \Omega(\xx) \) for \( \nsize \geq \CONSTn \)
\begin{EQ}[rcl]
%\label{1p1m1a1emxrrasde}
	\sup_{A \in \cc{B}(\R^{\dimp})}
	\left| 
		\P\bigl( \vupsv_{\GP} - \tilde{\upsv}_{\GP} \in A \cond \Xv \bigr)
		- \PG\bigl( \DPGPt^{-1} \gammav \in A \bigr)  
	\right|
%	\\
	& \leq &
	\CONST\, \nsize^{(1 - \smpa) / (2\smpa + 1)} \, ,
%	\CONST \, \rrGP^{3} \, \nsize^{-1/2} .
	\\
\label{1p1m1a1emxrrde}
%	\\
	\sup_{A \in \cc{B}_{\smp}(\R^{\dimp})}
	\left| 
		\P\bigl( \vupsv_{\GP} - \tilde{\upsv}_{\GP} \in A \cond \Xv \bigr)
		- \PG\bigl( \DPGPt^{-1} \gammav \in A \bigr)  
	\right|
%	\\
	& \leq &
	\CONST\, \nsize^{(2 - 2 \smpa) / (2\smpa + 1)} \, .
	\qquad
%	\CONST\, \rrGP^{6} \,  \nsize^{-1} \, ,
\end{EQ}
\end{theorem}

\begin{proof}
We proceed similarly to Theorem~\ref{CGLMlossGP} and Theorem~\ref{PGLMlossGPg}. 
Let \( \mmps \) be given by \eqref{6drvjhggv74e3ujf6hgewt}.
Then \( \dimL(\upsv) \asymp \mmps = (\CGPa \nsize)^{1/(2\smpa+1)} \) yielding \eqref{poybf3679jd532ff2st} for \( \nsize \geq \CONSTn \).
For validity of Laplace approximation \eqref{scdugfdwyd2wywy26e6de432} in Theorem~\ref{TBvMgen34},
we have to only check an addition condition \eqref{0hcde4dftedrf94yr5twew}.
It can be spelled out as \( \mmps^{3} \ll \nsize \).
For \( \smpa > 1 \), it is fulfilled automatically if \( \nsize \) is sufficiently large.
Bounds in \eqref{1p1m1a1emxrrde} are obtained from \eqref{scdugfdwyd2wywy26e6de432} by using \( \dimLt \asymp \mmps \).
\end{proof}
}{}

